CSOT: Curriculum and Structure-Aware Optimal Transport for Learning with Noisy Labels

Learning with noisy labels (LNL) poses a significant challenge in training a well-generalized model while avoiding overfitting to corrupted labels. Recent advances have achieved impressive performance by identifying clean labels and correcting corrupted labels for training. However, the current approaches rely heavily on the model's predictions and evaluate each sample independently without considering either the global and local structure of the sample distribution. These limitations typically result in a suboptimal solution for the identification and correction processes, which eventually leads to models overfitting to incorrect labels. In this paper, we propose a novel optimal transport (OT) formulation, called Curriculum and Structure-aware Optimal Transport (CSOT). CSOT concurrently considers the inter- and intra-distribution structure of the samples to construct a robust denoising and relabeling allocator. During the training process, the allocator incrementally assigns reliable labels to a fraction of the samples with the highest confidence. These labels have both global discriminability and local coherence. Notably, CSOT is a new OT formulation with a nonconvex objective function and curriculum constraints, so it is not directly compatible with classical OT solvers. Here, we develop a lightspeed computational method that involves a scaling iteration within a generalized conditional gradient framework to solve CSOT efficiently. Extensive experiments demonstrate the superiority of our method over the current state-of-the-arts in LNL. Code is available at https://github.com/changwxx/CSOT-for-LNL.

==> fig/analysis.tex <==
\begin{figure}[h]
  \centering
  \begin{subfigure}{0.3\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig/files/labeled_acc.pdf}
    \caption{Clean accuracy}
    \label{fig:clean_accuracy}
  \end{subfigure}
  % \hfill
  \begin{subfigure}{0.3\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig/files/unlabeled_acc.pdf}
    \caption{Corrected accuracy}
    \label{fig:corrected_accuracy}
  \end{subfigure}
  % \hfill
  \begin{subfigure}{0.3\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig/files/recall_rate.pdf}
    \caption{Clean recall rate}
    \label{fig:recall_rate}
  \end{subfigure}
  % \hfill
  % \begin{subfigure}{0.24\linewidth}
  %   \centering
  %   \scalebox{1.0} {\includegraphics[width=\linewidth]{fig/files/confusion_matrix.pdf}}
  %   \caption{}
  % \end{subfigure}
  \caption{Performance comparison for clean label identification and corrupted label correction.}
  \label{fig:subfigures}
\end{figure}



==> fig/curriculum_figure.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=1.\columnwidth]{fig/files/curriculum_v1.pdf}
\end{center}
\vspace{-0.3em}
\caption{An overview of curriculum denoise relabeling in binary classification case.}
\label{fig:curriculum}
\vspace{-1.2em}
\end{figure*}

==> fig/main_figure.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=1.\columnwidth]{fig/files/main.pdf}
\end{center}
\caption{
% 
\textbf{main.}
}
\label{fig:main}
\end{figure*}

==> fig/pseudo-labeling.tex <==
\begin{figure}
\centering
\includegraphics[width=1.\columnwidth]{fig/files/pseudo-labeling.pdf}
\caption{\textbf{pseudo-labeling comparison.}}
\label{fig:pseudo-labeling}
\vspace{-1.2em}
\end{figure}

==> formula/NC_OT_PL.tex <==
% \vspace*{1\baselineskip}
\begin{equation}
    \label{eq:NCOTPL}
    \min_{\mathbfQ\in\mathbfPi(\frac{1}{B}\ones_{B},
        \frac{1}{C}\ones_{C})}
        \tikzmarknode{class}{
            \highlight{red}{
                \left<-\log\mathbfP, \mathbfQ\right>
            }
        }
        +\kappa
            \left(
            \tikzmarknode{NCP}{\highlight{teal}{
            \Omega^{\mathbfP}(\mathbfQ)
            }} 
            + 
            \tikzmarknode{NCL}{\highlight{blue}{
            \Omega^{\mathbfL}(\mathbfQ)
            }}
            \right),
\end{equation}

\begin{tikzpicture}[overlay,remember picture,>=stealth,nodes={align=left,inner ysep=1pt},<-]
    % Label for class
    \path (class.north) ++ (0.6,0.8em) node[anchor=south east,color=red!65] (classtext){prediction certainty};
    \draw [color=red!85](class.north) |- ([xshift=-0.3ex,color=red!85]classtext.south west);

    % Label for NCP
    \path (NCP.south) ++ (-4.9,-0.2em) node[anchor=north west,color=teal!65] (NCPtext){prediction-level local consistency};
    \draw [color=teal!85](NCP.south) |- ([xshift=-0.3ex,color=teal!85]NCPtext.south west);
     % Label for NCL
    \path (NCL.south) ++ (-0,-0.4em) node[anchor=north west,color=blue!65] (NCLtext){label-level local consistency};
    \draw [color=blue!85](NCL.south) |- ([xshift=-0.3ex,color=blue!85]NCLtext.south east);
\end{tikzpicture}
% \vspace*{1\baselineskip}


==> formula/curriculum_allocator.tex <==

\begin{equation}
    \label{eq:curriculum_allocator}
    \min_{\mathbfQ}
        % \tikzmarknode{class}{\highlight{red}{
                \left<-\log\mathbfP, \mathbfQ\right>
            % }}
        +\kappa
            \left(
            % \tikzmarknode{NCP}{\highlight{teal}{
            \Omega_{\text{NC}}^{\mathbfP}(\mathbfQ)
            % }} 
            + 
            % \tikzmarknode{NCL}{\highlight{blue}{
            \Omega_{\text{NC}}^{\mathbfL}(\mathbfQ)
            % }}
            \right)
\end{equation}
\vspace*{1\baselineskip}
\begin{equation*}
\text{s.t.} \quad
\mathbfQ \in 
\left\{\mathbfQ\in\mathbb{R}_{+}^{B \times C}
        |\mathbfQ\ones_{C}\leq\frac{1}{B}\ones_{B},
        \mathbfQ^\top\ones_{B}=\frac{m}{C}\ones_{C}
        \right\}.
\end{equation*}


% \begin{tikzpicture}[overlay,remember picture,>=stealth,nodes={align=left,inner ysep=1pt},<-]
%     % Label for class
%     \path (class.north) ++ (0.6,0.8em) node[anchor=south east,color=red!65] (classtext){prediction certainty score};
%     \draw [color=red!85](class.north) |- ([xshift=-0.3ex,color=red!85]classtext.south west);

%     % Label for NCP
%     \path (NCP.south) ++ (-3.9,-0.2em) node[anchor=north west,color=teal!65] (NCPtext){prediction-level NC score};
%     \draw [color=teal!85](NCP.south) |- ([xshift=-0.3ex,color=teal!85]NCPtext.south west);
%      % Label for NCL
%     \path (NCL.south) ++ (-0,-0.4em) node[anchor=north west,color=blue!65] (NCLtext){label-level NC score};
%     \draw [color=blue!85](NCL.south) |- ([xshift=-0.3ex,color=blue!85]NCLtext.south east);
% \end{tikzpicture}
% \vspace*{1\baselineskip}


==> tab/CSOT_timecost.tex <==
\begin{table}
\centering
\caption{\textbf{Time cost (s) for solving CSOT optimization problem of different input sizes.}
VDA indicates vanilla Dykstra’s algorithm-based CSOT solver, while ESI indicates efficient scaling iteration-based solver.
}
\label{tab:CSOT_timecost}
\resizebox{0.5\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{lcc} 
\toprule
$(|\bmAlpha|,|\bmBeta|)$ & VDA-based & ESI-based (Ours)  \\ 
\hline
(1024,10)                & 0.83        & \textbf{0.82} \textcolor{red}{$\downarrow$}         \\
(1024,50)                & 1.00        & \textbf{0.80} \textcolor{red}{$\downarrow$}         \\
(1024,100)               & 0.87        & \textbf{0.80} \textcolor{red}{$\downarrow$}         \\ 
\hline
(50,50)                  & 0.82        & \textbf{0.79} \textcolor{red}{$\downarrow$}         \\
(100,100)                & 0.88        & \textbf{0.80} \textcolor{red}{$\downarrow$}         \\
(500,500)                & 0.88        & \textbf{0.87} \textcolor{red}{$\downarrow$}         \\
(1000,1000)              & 0.94        & \textbf{0.81} \textcolor{red}{$\downarrow$}         \\
(2000,2000)              & 2.11        & \textbf{0.98} \textcolor{red}{$\downarrow$}         \\
\textbf{(3000,3000)}              & 3.74        & \textbf{0.99} \textcolor{red}{$\downarrow$}         \\
\bottomrule
\end{tabular}
} %< \resizebox
\end{table}

==> tab/cifar_v0.tex <==
\begin{table}
\centering
\caption{\textbf{Comparison with state-of-the-art methods in test accuracy (\%) on CIFAR-10 and CIFAR-100.} 
The results are mainly copied from \cite{NCE,RRL}.
We present the performance of our CSOT method using the "mean$\pm$variance" format, which is obtained from 3 trials with different seeds.}
\label{tab:cifar}
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{r|ccccc|cccc}
\toprule
Dataset                                           & \multicolumn{5}{c|}{CIFAR-10}                                                                                                                                                                                                                                                                                                           & \multicolumn{4}{c}{CIFAR-100}                                                                                                                                                                                                                                 \\
Noise type                                        & \multicolumn{4}{c}{Symmetric}                                                                                                                                                                                                                                         & Assymetric                                                      & \multicolumn{4}{c}{Symmetric}                                                                                                                                                                                                                                 \\
Method/Noise ratio                                & 0.2                                                             & 0.5                                                             & 0.8                                                             & 0.9                                                             & 0.4                                                             & 0.2                                                    & 0.5                                                             & 0.8                                                             & 0.9                                                              \\ 
\midrule
Cross-Entropy                                     & 86.8                                                            & 79.4                                                            & 62.9                                                            & 42.7                                                            & 85.0                                                            & 62.0                                                   & 46.7                                                            & 19.9                                                            & 10.1                                                             \\
F-correction \cite{F-correction} & 86.8                                                            & 79.8                                                            & 63.3                                                            & 42.9                                                            & 87.2                                                            & 61.5                                                   & 46.6                                                            & 19.9                                                            & 10.2                                                             \\
Co-teaching+ \cite{Co-teaching}  & 89.5                                                            & 85.7                                                            & 67.4                                                            & 47.9                                                            & -                                                               & 65.6                                                   & 51.8                                                            & 27.9                                                            & 13.7                                                             \\
PENCIL \cite{PENCIL}             & 92.4                                                            & 89.1                                                            & 77.5                                                            & 58.9                                                            & 88.5                                                            & 69.4                                                   & 57.5                                                            & 31.1                                                            & 15.3                                                             \\
DivideMix \cite{DivideMix}       & 96.1                                                            & 94.6                                                            & 93.2                                                            & 76.0                                                            & 93.4                                                            & 77.3                                                   & 74.6                                                            & 60.2                                                            & 31.5                                                             \\
ELR \cite{ELR}                   & 95.8                                                            & 94.8                                                            & 93.3                                                            & 78.7                                                            & 93.0                                                            & 77.6                                                   & 73.6                                                            & 60.8                                                            & 33.4                                                             \\
NGC \cite{NGC}                   & 95.9                                                            & 94.5                                                            & 91.6                                                            & 80.5                                                            & 90.6                                                            & 79.3                                                   & 75.9                                                            & 62.7                                                            & 29.8                                                             \\
RRL \cite{RRL}                   & 96.4                                                            & 95.3                                                            & 93.3                                                            & 77.4                                                            & 92.6                                                            & 80.3                                                   & 76.0                                                            & 61.1                                                            & 33.1                                                             \\
MOIT \cite{MOIT}                 & 93.1                                                            & 90.0                                                            & 79.0                                                            & 69.6                                                            & 92.0                                                            & 73.0                                                   & 64.6                                                            & 46.5                                                            & 36.0                                                             \\
OTCleaner \cite{OTCleaner}       & 91.4                                                            & 85.4                                                            & 56.9                                                            & -                                                               & -                                                               & 67.4                                                   & 58.9                                                            & 31.2                                                            & -                                                                \\
NCE \cite{NCE}                   & 96.2                                                            & 95.3                                                            & 93.9                                                            & 88.4                                                            & 94.5                                                            & \textbf{81.4}                                          & 76.3                                                            & 64.7                                                            & 41.1                                                             \\ 
\midrule
\textbf{CSOT (Best)}                              & \textbf{96.6\tiny{$\pm$0.10}} & \textbf{96.2\tiny{$\pm$0.11}} & \textbf{94.4\tiny{$\pm$0.16}} & \textbf{90.7\tiny{$\pm$0.33}} & \textbf{95.5\tiny{$\pm$0.06}} & 80.5\tiny{$\pm$0.28} & \textbf{77.9\tiny{$\pm$0.18}} & \textbf{67.8\tiny{$\pm$0.23}} & \textbf{50.5\tiny{$\pm$0.46}}  \\
\textbf{CSOT (Last)}                              & 96.4\tiny{$\pm$0.18}          & 96.0\tiny{$\pm$0.11}          & 94.3\tiny{$\pm$0.20}          & 90.5\tiny{$\pm$0.36}          & 95.2\tiny{$\pm$0.12}          & 80.2\tiny{$\pm$0.31} & 77.7\tiny{$\pm$0.14}          & 67.6\tiny{$\pm$0.36}          & 50.3\tiny{$\pm$0.33}           
\\ \bottomrule
\end{tabular}
} %< \resizebox
\end{table}
